PEM: Representing Binary Program Semantics for Similarity Analysis via a Probabilistic Execution Model

Binary similarity analysis determines if two binary executables are from the same source program. Existing techniques leverage static and dynamic program features and may utilize advanced Deep Learning techniques. Although they have demonstrated great potential, the community believes that a more effective representation of program semantics can further improve similarity analysis. In this paper, we propose a new method to represent binary program semantics. It is based on a novel probabilistic execution engine that can effectively sample the input space and the program path space of subject binaries. More importantly, it ensures that the collected samples are comparable across binaries, addressing the substantial variations of input specifications. Our evaluation on 9 real-world projects with 35k functions, and comparison with 6 state-of-the-art techniques show that PEM can achieve a precision of 96% with common settings, outperforming the baselines by 10-20%.

==> fig_attention.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{.31\textwidth}
        \begin{minipage}{\textwidth}
        \includegraphics[width=\textwidth]{figs/cat-O3-instrs.pdf}
        \end{minipage}
        \caption{cat O3}
    \end{subfigure}
    \rulesep
    \begin{subfigure}[b]{.31\textwidth}
        \includegraphics[width=\textwidth]{figs/cat-O0-instrs.pdf}
        \caption{cat O0}
    \end{subfigure}
    \rulesep
    \begin{subfigure}[b]{.31\textwidth}
        \includegraphics[width=\textwidth]{figs/touch-O0-instrs.pdf}
        \caption{touch O0}
    \end{subfigure}
    \caption{Visualized Attention Layers of SAFE (Darker Color Means Higher Weight)}
    \label{fig:apdx:att}
    \vspace{-5pt}
\end{figure*}

==> fig_baseline2-2.tex <==

\begin{figure}[H]
    \centering
    \includegraphics[width=.40\textwidth]{figs/eval/ratio-perf.pdf}
    
    \caption{
    Variation of PR@1 w.r.t. Negative Sample Ratios. Each figure presents results for one pair of binaries in Dataset-\MakeUppercase{\romannumeral 2}. The $x$ axes denote different ratios of negative samples over positive samples, from 1:1 to $\infty$:1, where $\infty$ is the number of all functions in the binary file. The $y$ axes denote PR@1. Blue, orange, green lines depict performance of \toolname, SAFE, and Trex, respectively.
    }
    \label{fig:baseline2-2}
\end{figure}

==> fig_cfgs.tex <==
\begin{figure*}
\centering
\begin{subfigure}[b]{.26\textwidth}
    \includegraphics[width=\textwidth]{figs/cfg-cat3.pdf}
    \vspace{-20pt}
    \caption{Cat@O3 (144 blocks and 218 edges)}
    \label{fig:cfg:cat3}
\end{subfigure}
\hspace{.01\textwidth}
\begin{subfigure}[b]{.26\textwidth}
    \includegraphics[width=\textwidth]{figs/cfg-cat0.pdf}
    \vspace{-20pt}
    \caption{Cat@O0 (83 blocks and 144 edges)}
    \label{fig:cfg:cat0}
\end{subfigure}
\hspace{.01\textwidth}
\begin{subfigure}[b]{.26\textwidth}
    \includegraphics[width=\textwidth]{figs/cfg-touch0.pdf}
    \vspace{-20pt}
    \caption{\textls[-20]{Touch@O0\,(89\,blocks~and~120\,edges)}}
    \label{fig:cfg:touch0}
\end{subfigure}

    \caption{Control-Flow-Graphs for Motivation Examples
    }
    \label{fig:cfgs}
    \vspace{-17pt}
\end{figure*}

==> fig_dist_expectation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.6\linewidth]{figs/method/effect-of-k-exp.pdf}    
    \caption{$\mathbf{E}(\prmath(i))$ w.r.t. $K$. The $x$ axis denotes the value of $K$ (i.e., the total number of additional samplings). The $y$ axis denotes the value of $\mathbf{E}(\prmath(i))$ (i.e., the expectation of reward)}
    \label{fig:effect-k-exp}

    
\end{figure}

==> fig_dist_k.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figs/method/mutation_path.pdf}
    \caption{Distribution of $k$. The $x$-axis denotes the number of flipped predicates on a path. The $y$-axis denotes the number of paths. The blue curve depicts the number of all $x$-edge-off paths. The orange curve denotes the number of coincided paths. It is obtained by multiplying each point on the blue curve with $\mathcal{P}_{same}(x)$.
    }
    \label{fig:k-off-dist}
\end{figure}

==> fig_dist_path_sim.tex <==
\begin{figure*}[t]
\begin{subfigure}[t]{.4\textwidth}
    \includegraphics[width=\textwidth]{figs/method/path_similarity_scatter.pdf}
    \caption{The $x$-axis denotes functions, whose names are elided. The $y$-axis denotes the similarity score of paths in the {\tt -O0} function to the most similar path in the {\tt -O3} function. Green and orange points denote paths from similar and dissimilar pairs.}
    \label{fig:path-sim-scatter}
\end{subfigure}
\hspace{10pt}
\begin{subfigure}[t]{.4\textwidth}
    \includegraphics[width=\textwidth]{figs/method/path_similarity_hist.pdf}
    \caption{The $x$-axis denotes the similarity score of paths from the {\tt -O0} function to the most similar path from the {\tt -O3} function. The $y$-axis denotes the frequency of paths. Green and orange bars denote distributions of similar and dissimilar pairs.}
    \label{fig:path-sim-hist}
\end{subfigure}
    \caption{Distribution of Path Similarity. Fig.~\ref{fig:path-sim-scatter} shows
    paths from similar and dissimilar pairs w.r.t. functions; Fig.~\ref{fig:path-sim-hist} aggregates the distribution of  similarity scores.}
    \label{fig:path-sim}    
    \vspace{-2pt}
\end{figure*}

==> fig_eva_branch_dist.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.4\textwidth]{figs/eval/branch-dist.pdf}
    \vspace{-1pt}
    \caption{ \revise{\textls[-5]{Correspondence of Predicates with Min and Max Selectivity.
    Blue is for min and orange for max. For example, the bar at min+1 means that about 20 predicates with min selectivity in one trace have min+1 selectivity in the other~trace.} }
    }
    \label{fig:branch-dist}
    \vspace{-10pt}
\end{figure}

==> fig_eva_branch_relation.tex <==
\begin{figure}[t]
\vspace{-5pt}
    \centering
    \includegraphics[width=.31\textwidth]{figs/eval/branch-relation.pdf}
    \vspace{-3pt}
    \caption{\revise{Predicate Correspondence versus Dynamic Selectivity.
    Each blue dashed line represents the analysis results of path pairs from two respective binaries compiled differently from a program.
The $x$ axis represents selectivity (with {\it min} the minimal and {\it max} the maximum) and $y$ denotes the percentage of predicate matches. %
We also compute the median for each selectivity, %
 resulting in the orange line.} %
}
    \label{fig:branch-relation}
    \vspace{-3pt}
\end{figure}


==> fig_eva_coverage.tex <==
\begin{figure}[t]
\vspace{-5pt}
    \centering
    \includegraphics[width=.43\textwidth]{figs/eval/coverage.pdf}
    \vspace{-4pt}
    \caption{Coverage of \toolname 
    }
    \label{fig:Coverage}
    \vspace{-3pt}
\end{figure}

==> fig_eva_how_solve.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.98\linewidth]{figs/eval/how-solve.pdf}
    \vspace{-3pt}
    \caption{\textls[-20]{Comparison with How-Solve. We leverage the best two models (i.e., GNN and GMN) in How-Solve. Each bar denotes a program, whose name is elided. 
    A bar with 1.0 PR@1 means that \toolname finds the correct matches for all functions in the program. 
    Dashed lines denote the average PR@1 of each tool.}
    } 
    \label{fig:how-help}
    \vspace{-1pt}
\end{figure}

==> fig_logging_rules.tex <==
\begin{figure}[t]
\begin{mdframed}
\begin{minipage}{\textwidth}
{\footnotesize
\begin{mathpar}
\inferrule{Regs[r_2]=a\\ \textbf{valid}(a) \\ v=M[a]\\ OV'=\update{OV}{a}{OV[a]+1}\\
OV''=\update{OV'}{v}{OV'[v]+1}\\
}
{\progstate{Regs}{r_1 = [r_2];I}{ic}{M}{OV}
\\ \\ \\ \\ \rightarrow
\progstate{Regs}{r_1 = [r_2];I}{ic}{M}{OV''}
}
{LogLd}\\
\inferrule{Regs[r_2]=a\\ \neg\textbf{valid}(a) \\  v=\textbf{invalidLd}(a)\\ \\ \\ \\ OV'=\update{OV}{a}{OV[a]+1}\\ \\ \\ \\ \\ \\ \\ \\
OV''=\update{OV'}{v}{OV'[v]+1}\\
}
{\progstate{Regs}{r_1 = [r_2];I}{ic}{M}{OV}
\\ \\ \\ \\ \rightarrow
\progstate{Regs}{r_1 = [r_2];I}{ic}{M}{OV''}
}
{LogIvLd}\\
\inferrule{Regs[r_1]=a\\ Regs[r_2]=v\\ \\ \\ \\ \\ 
OV'=\update{OV}{a}{OV[a]+1}\\ \\ \\ \\ \\ \\ \\ 
OV''=\update{OV'}{v}{OV'[v]+1}
}
{\progstate{Regs}{[r_1] = r_2;I}{ic}{M}{OV}
 \rightarrow\\
\progstate{Regs}{[r_1] = r_2;I}{ic}{M}{OV''}
}
{LogSt}\\
\inferrule{
OV'=\update{OV}{a}{OV[a]+1}\\
}
{\progstate{Regs}{\langkw{jmp}\ a;I}{ic}{M}{OV}
\rightarrow\\ \\
\progstate{Regs}{\langkw{jmp}\  a;I}{ic}{M}{OV'}
}
{LogJN}\\
\inferrule{Regs[r] = a\\
OV'=\update{OV}{a}{OV[a]+1}\\
}
{\progstate{Regs}{\langkw{jr}\ r;I}{ic}{M}{OV}
\rightarrow
\progstate{Regs}{\langkw{jr}\ r;I}{ic}{M}{OV'}
}
{LogJR}\\
\inferrule{Regs[r_2]=v_2\\ Regs[r_3]=v_3\\ \\ \\ 
v_1 = \textbf{condValue}(\otimes, v_2, v_3)\\
OV'=\update{OV}{v_1}{OV[v_1]+1}\\
}
{\progstate{Regs}{r_1 = r_2 \otimes r_3;I}{ic}{M}{OV} 
\\ \\ \\ \rightarrow
\progstate{Regs}{r_1 = r_2 \otimes r_3;I}{ic}{M}{OV'}
}
{LogCC}
\end{mathpar} 
} 
\end{minipage}
\label{fig:sem:rule_sem}
\end{mdframed}    
\caption{Logging Rules}
\label{fig:supp:logging}
\end{figure}

==> fig_mem_model.tex <==
\begin{figure}[t]
\begin{minipage}{\textwidth}
\begin{lstlisting}[deletekeywords={input}, style=customc, firstnumber=1, xleftmargin=0.5cm, basicstyle=\scriptsize,
    escapeinside={(|}{|)}]
struct DoubleList{
    /* offset 0x0 */ double val;
    /* offset 0x8 */ DoubleList* next;};
struct PointList{
    /* offset 0x0  */ int64 x,y;
    /* offset 0x10 */ PointList* next;};
DoubleList* findDouble(DoubleList* list, double val){ (|\label{line:ll:func}|)
    while(list){
        if(val == list->val) (|\label{line:ll:val}|)
            return list;
        list = list->next; (|\label{line:ll:next}|)
    }
    return list;
}
PointList* findPoint(PointList* list, int64 x, int64 y){ (|\label{line:ll:func}|)
    while(list){
        ...
        list = list->next; (|\label{line:ll:next}|)
    } ...
}
\end{lstlisting}
\end{minipage}
\vspace{-5pt}
\caption{Example Illustrating Probabilistic Memory Model}
\label{fig:mem-model}
\end{figure}


==> fig_motivation.tex <==
\begin{figure}[t!]
\begin{subfigure}[b]{.48\textwidth}
\begin{minipage}{\textwidth}
\begin{lstlisting}[deletekeywords={input}, style=customc, firstnumber=1, xleftmargin=0.5cm, basicstyle=\scriptsize,
    escapeinside={(|}{|)}]
void main_cat(int argc, char** argv){
    while(-1!=(c=get_cli_opt(argc, argv, "bestuv"))){ (|\label{line:cat:cli0}|)
        switch(c){ (|\label{line:cat:switch}|)
            case 'b': flag0 = true; ...; format = true; break; (|\label{line:cat:f0}|)
            case 'e': flag1 = true; break;
            case 'v': print("Coreutils v8.30"); break;
            ...
            default: quote("error"); abort(); (|\label{line:cat:error}|)
        }
    }(|\label{line:cat:cli1}|)
    ...//define: (|\texttt{pageSize, inbuf}|) and (|\texttt{insize}|)  (|\label{line:cat:define}|)
    do{(|\label{line:cat:print0}|)
        if((flag0||flag1) && format){ (|\label{line:cat:condi}|)
            ret = simple_cat(inbuf, insize); (|\label{line:cat:simple}|)
        }else{ ...
            outbuf = xmalloc(outbuf, pageSize) (|\label{line:cat:malloc}|)
            ret = complex_cat(inbuf, insize, outbuf); (|\label{line:cat:complex}|)
        }
    }while(...);(|\label{line:cat:while}|)(|\label{line:cat:print1}|)
}
int complex_cat(char* inbuf, int insize, char* outbuf){
    if(print_invisible && inbuf[i]<0x20) (|\label{line:cat:print-inv}|)
        outbuf[...] = to_ascii(inbuf[i])
}
\end{lstlisting}
\end{minipage}
\vspace{-15pt}
\caption{Coreutils: cat}
\vspace{-3pt}
\label{fig:src:cat}
\end{subfigure}

\begin{subfigure}[b]{.48\textwidth}
\begin{minipage}{\textwidth}
\begin{lstlisting}[deletekeywords={input}, style=customc, firstnumber=1, xleftmargin=0.5cm, basicstyle=\scriptsize,
    escapeinside={(|}{|)}]
void main_touch(int argc, char** argv){
    while(-1!=(c=get_cli_opt(argc, argv, "bcdfhv"))){ (|\label{line:touch:optbegin}|)
        switch(c){ (|\label{line:touch:switch}|)
            case 'b': flag |= 0x100; break;
            case 'c': flag = 0x1; break;
            case 'v': print("Coreutils v8.30"); break;
            ...
            default: quote("error"); abort(); (|\label{line:touch:error}|)
        }
    }(|\label{line:touch:optend}|)
    for(int i = begin; i < argc; i++) (|\label{line:touch:touchbegin}|)
        touch_function(argv[i]); (|\label{line:touch:touchfunc}|)
    
}
\end{lstlisting}
\end{minipage}
\vspace{-20pt}
\caption{Coreutils: touch}
\label{fig:src:touch}
\end{subfigure}
  \caption{%
  Motivating Example
  }
  \label{fig:moti_ex}
\end{figure}


==> fig_pm_region.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.40\textwidth]{figs/mem.pdf}
    \caption{Example of Probabilistic Memory Region. The numbers on the top denote the lowest 4 bits of memory addresses, and the numbers on the left denote the highest 8 bits. Cells with bold texts are the least significant byte (LSB). 
    Memory cells in blue are exclusively accessed by {\tt findDouble} and those in red are exclusively accessed by {\tt findPoint}. Green cells are accessed by both functions and white cells are accessed by neither. Also, cells in bold boxes
    are interpreted as pointers, with arrows pointing to their targets.}
    \label{fig:PM-region}
\end{figure}

==> fig_rules.tex <==
\newcommand{\update}[3]{\ensuremath{#1[#2\rightsquigarrow#3]}\xspace}
\newcommand{\progstate}[5]{\ensuremath{\langle #1,#2,#3,#4,#5\rangle}\xspace}
\begin{figure}[t]
\begin{mdframed}
\begin{minipage}{\textwidth}
{\footnotesize
\vspace{-3pt}
\boxed{\textbf{State Configuration:}\  \progstate{Regs}{I}{ic}{M}{OV}} \\
\vspace{-3pt}
\begin{mathpar}
\inferrule{\texttt{EntryPoint} = en\\ \forall r, Regs[r]=s
}
{\progstate{\emptyset}{\emptyset}{0}{\emptyset}{\emptyset}
\rightarrow
\progstate{Regs}{\textbf{decode}(en)}{1}{\emptyset}{\emptyset}
}
{Start}\\
\vspace{-3pt}
\inferrule{
p[ic]=a' \\ I'=\textbf{decode}(a')
}
{\progstate{Regs}{\langkw{jcc}\ r\ a;I}{ic}{M}{OV}
\rightarrow
\progstate{Regs}{I'}{ic+1}{M}{OV}
}
{JccGT}\\
\vspace{-3pt}%
\inferrule{Regs[r]\ne 0\\ p[ic]=\bot \\ I'=\textbf{decode}(a)}
{\progstate{Regs}{\langkw{jcc}\ r\ a;I}{ic}{M}{OV}
\rightarrow
\progstate{Regs}{I'}{ic+1}{M}{OV}
}
{JccT}\\
\vspace{-3pt}
\inferrule{Regs[r]=0 \\ p[ic]=\bot}
{\progstate{Regs}{\langkw{jcc}\ r\ a;I}{ic}{M}{OV}
\rightarrow
\progstate{Regs}{I}{ic+1}{M}{OV}
}
{JccF}\\
\vspace{-3pt}
\inferrule{Regs[r_2]=a\\  v=M[a]\\ Regs'=\update{Regs}{r_1}{v}}
{\progstate{Regs}{r_1 = [r_2];I}{ic}{M}{OV}
\rightarrow
\progstate{Regs'}{I}{ic+1}{M}{OV}
}
{LdV}\\
\vspace{-3pt}
\inferrule{Regs[r_2]=a\\ \textbf{valid}(a) \\ M[a]=\bot\\ Regs'=\update{Regs}{r_1}{s}}
{\progstate{Regs}{r_1 = [r_2];I}{ic}{M}{OV}
\rightarrow
\progstate{Regs'}{I}{ic+1}{M}{OV}
}
{LdUd}\\
\vspace{-3pt}
\inferrule{Regs[r_2]=a\\ \neg\textbf{valid}(a) \\
v=\textbf{invalidLd}(a)\\
Regs'=\update{Regs}{r_1}{v}}
{\progstate{Regs}{r_1 = [r_2];I}{ic}{M}{OV}
\rightarrow
\progstate{Regs'}{I}{ic+1}{M}{OV}
}
{LdIv}
\end{mathpar}
} %
\end{minipage}
\label{fig:sem:rule_exec}
\end{mdframed}    
\caption{Interpretation Rules 
}
\label{fig:sem_rule}
\vspace{-3pt}
\end{figure}




==> fig_syntax.tex <==
\begin{figure}[t]
\vspace{-5pt}
    \begin{mdframed}
      {\footnotesize \tt
        \addtolength{\tabcolsep}{-5pt}
  \begin{grammar}
    <\texttt{Program}> $P$ $\Coloneqq$ $I$
\ \ 
    $\langle\texttt{Register}\rangle$ $R$ $\Coloneqq$ $\{r_0, r_1, \dots, r_{31}\}$  \vspace{-5pt}
    
    <\texttt{Val}> $v$ $\Coloneqq$ $\{0, 1, 2, ...\}$
    $\;\;\;\;\;\;\;\;\;\;\;\;\;$
    $\langle\texttt{Addr}\rangle$ $a$ $\Coloneqq$ $\{0, 1, 2, ...\}$
    \vspace{-5pt}
    
    <\texttt{Comparison}> $\otimes$ $\Coloneqq$ $\{==, \ge, \le, \dots\}$ \;\;\;\;
    $\langle\texttt{BinOp}\rangle$ $\diamond$ $\Coloneqq$ $\{+, -, *, \dots\}$
    \vspace{-5pt}
    
    <\texttt{Instruction}> $I$ $\Coloneqq$ $r_1=r_2$|$r = v$|$r_1 = r_2 \otimes r_3$|$r_1 = r_2 \diamond r_3$ 
    \alt $r_1 = [r_2]$ | $[r_1] = r_2$  | $\langkw{jmp}\ a$ | $\langkw{jcc}\ r\ a$ | $\langkw{jr}\ r$
    | $\langkw{done}$
    | $I_1;I_2$
    
  \end{grammar}
      }
    \end{mdframed}
    \caption{Syntax of Our Language}
    \label{fig:definition}
    \vspace{-16pt}
\end{figure}

==> fig_sys_abl.tex <==
\begin{figure}[t]
    \centering    
    \begin{subfigure}[t]{.2\textwidth}
        \includegraphics[width=\textwidth]{figs/eval/abl-loop.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{.2\textwidth}
        \includegraphics[width=\textwidth]{figs/eval/abl-str.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{.2\textwidth}
        \includegraphics[width=\textwidth]{figs/eval/abl-mem.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{.2\textwidth}
        \includegraphics[width=\textwidth]{figs/eval/abl-ins.pdf}
    \end{subfigure}        
    \caption{Perf. w.r.t. Different Configurations. Each sub-figure presents the experimental results of changing one system configuration. The $x$ axes denote different values of the related system configurations, and the $y$ axes denote the values for  the metrics. The blue lines represent  PR@1, the orange lines  coverage for -O0 programs, and the green lines  coverage for -O3 programs.}
    \label{fig:sys-abl}
\end{figure}

==> fig_tex/fig_effect_prob_sample.tex <==
% \begin{figure}[t]
%     \centering
% \begin{subfigure}[t]{.24\textwidth}
%         \includegraphics[width=\textwidth]{figs/method/effect-of-k-dist.pdf}
%         \vspace{-20pt}
%         \caption{\revise{Dist. of $i$ with Different $K$}}
%         % \label{fig:effect-k-dist}
% \end{subfigure}
% \begin{subfigure}[t]{.24\textwidth}
%         \includegraphics[width=\textwidth]{figs/method/effect-of-k-exp.pdf}
%         \vspace{-20pt}
%         \caption{\revise{$\mathbf{E}(\mathcal{R}(i))$ w.r.t. $K$}}
%         % \label{fig:effect-k-exp}
% \end{subfigure}
%     \caption{\xx{Old Figure.}Effects of Probabilistic Sampling. In \ref{fig:effect-k-dist}, the $x$ axis denotes the number of correct steps, and the $y$ axis denotes the probability $\widetilde{PC}(i, B-i)$
%     \xz{is it $\widetilde{PC}(i, B-i)$? you introduce a new P(i) and it is unclear how that is computed. If so, you need to fix the symbol in the text as well\xx{}}. 
%     The blue line is for $K=0$ and the orange line is for $K=80$. In \ref{fig:effect-k-exp}, the $x$ axis denotes different value of $K$ and the $y$ axis denotes the expected value of $\mathcal{R}(i)$ with the related $K$.}
    
%     \label{fig:effect-prob-sample}
%     \vspace{-3pt}
% \end{figure}

==> fig_time_eff.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=.29\textwidth]{figs/eval/time-boxplot.pdf}
    \caption{Efficiency %
    The left depicts the throughput for interpretation and preprocessing.
The $y$ axis is the number of functions \toolname can process per second. We can see that \toolname analyzes more than 3 functions per second in most cases.
The right part depicts the throughput for comparison. It illustrates that 
\toolname compares more than 2000 pairs per second in most cases.
    }
    \label{fig:time-eff}
\end{figure}

==> old-ablation.tex <==
\vspace{-5pt}
\subsection{Ablation Study}

We perform three ablation studies to see how each part of our system contributes to the comparison result. We perform all the ablation study on the main functions of {\it Coreutils}. We run \toolname with different configurations and calculate the PR@1 and coverage. We find that the probabilistic path sampling algorithm effectively selects consistent paths from the optimized and unoptimized version of binaries. Also, our probabilistic execution model is robust under different sets of seed values. We further find that the matched values (i.e., values that we see in both the optimized and the unoptimized binaries) have similar frequency before and after optimization. More can be found in our supplementary document~\cite{sup-docs}. 


==> old-eval.tex <==

\toolname is developed on QEMU. 
We evaluate its performance via three research questions:\\
\textbf{RQ1:} How does \toolname perform compared to the baselines?\\
\textbf{RQ2:} How does the performance of different tools vary with different data compositions?\\
\textbf{RQ3:} How useful is \toolname in real-world applications? 

\subsection{Setup}

We conduct the experiments on a server running Ubuntu 18.04 equipped with a 24-core Intel(R) Xeon(R) Silver 4214R CPU at 2.40GHz, 188G memory, and 8 NVIDIA RTX A6000 GPUs.

\noindent
{\bf Datasets.} 
We use two datasets for our evaluation.

\noindent Dataset-\MakeUppercase{\romannumeral 1}: To compare with IMF and BLEX, which only use Coreutils as their dataset, we construct a dataset from Coreutils-8.32. We compile the dataset using two different compilers GCC-9.4 and Clang-12, with 3 optimization levels (i.e., O0, O2, O3). 

\noindent Dateset-\MakeUppercase{\romannumeral 2}: This dataset includes Coreutils-8.32, Curl-7.71.1, Diffutils 3.7, Findutils-4.7.0, OpenSSL-1.0.1f, SQLite-3.34.0,  ImageMagick-7.0.10, and Zlib-1.2.11, which are commonly used by Trex\cite{trex} and How-Solve\cite{How-Solve}. The binaries are obtained from the GitHub repository of Trex\cite{trex}. We do not include Libmicrohttpd and LibTomCrypt as they cannot be executed.
We use the same 3 optimization levels. 


\noindent
{\bf Baseline Tools.} 
We choose 2 kinds of state-of-the-art methods as the baselines.
We use two execution-based methods: IMF and BLEX (Baseline-I), which are SOTAs in this line as far as we know.
We also choose two Deep Learning methods (Baseline-II): SAFE and Trex. We use their pre-trained models or train using their released implementation and default hyper-parameters. 
We also compare with the reported results in How-Solve\cite{How-Solve} that conducts the first measurement study on how machine learning can be used to solve the binary function similarity problem. 


\noindent{\bf Metrics.} 
We use Precision at Position 1 (PR@1) as the metric. Given a function, PR@1 measures whether the matched function scores the highest out of a pool of target functions.
Many data-driven methods~\cite{binai,trex,safe,How-Solve} mainly use {\em Area Under Curve} (AUC) of the {\em Receiver Operating Characteristic} (ROC) curve to measure performance. While these data-driven methods achieve high AUC scores, existing literature~\cite{DoandDont} points out that a good AUC score does not necessarily imply good performance for a classifier on an imbalanced dataset (e.g., a class ratio of 1:100, class 1 having 1 sample and class 2 having 100). Therefore we choose precision at 1 as our metric. Intuitively, PR@1 matches the real-world use-scenario of binary similarity. For example, to detect one-day vulnerabilities, a tool should accurately detect the problematic function from others. 

The formula to calculate PR@1 is a specialized version of calculating PR@k, with $k=1$. Specifically, 
$
\mathit{PR@k} = \frac{\# \ \mathit{of} \ \mathit{match@k}}{\# \ \mathit{of} \ \mathit{queries}}
$, where
 $\# \ of \ queries$ means the number of times that we try to find a function most similar to the truth function; $\# \ of \ match@k$ means the number of times the true-positive is among the top $k$ functions.


    
 
 
 





\subsection{RQ1: Comparison to Baselines}
\label{sec:compare1}
\noindent{\bf Time Efficiency.}
On average, \toolname takes 0.14 seconds to interpret a function. It further takes 0.3 seconds to aggregate the observable values collected during interpretation. After that, we use Python scripts to perform value set comparisons. It on average compares 5,000  pairs per second using one CPU.  
When processing the same binary (i.e., Coreutils on Dataset-\MakeUppercase{\romannumeral 1}) as IMF and BLEX, 
\toolname takes 5 minutes to interpret the binary, 8 minutes to aggregate the result, and 5 minutes to compare every pair of functions in two Coreutils binaries and compute the similarity score. Note that it is a one-time effort to interpret the functions and aggregate observable values for all pairs.
In comparison, BLEX takes 1.2 CPU hours to process a binary (comparison not included) and IMF takes 0.52 hours to process and compare a pair of binaries. \toolname achieves significantly better time efficiency than BLEX and is more efficient than IMF, especially when taking the code coverage into consideration. 
Machine learning models typically have expensive training time. They have better performance in test time as they can leverage GPUs. 


\noindent{\bf Coverage.}
The code coverage of \toolname on Dataset-II is shown in Fig.~\ref{fig:Coverage}. The horizontal axis marks the projects and the vertical axis shows the percentage of functions for which \toolname has achieved various levels of coverage, denoted by different colors. As we can see, 80\% of the functions in {\tt O0} and 70\% functions in {\tt O3} have a full or close-to-full coverage. Those functions with less than 40\% coverage have extremely complex control flow structures. 
They typically have many inlined callees.
For example, the main function of {\it sort} in {Coreutils} has 496 basic blocks, resulting in  millions of potential paths. Note that even from such a huge path space, \toolname is still able to select similar paths and collect consistent values with a high probability.

\noindent{\bf Comparison to Baseline-\MakeUppercase{\romannumeral 1}.}
We compare \toolname with Baseline-\MakeUppercase{\romannumeral 1} on Dataset-\MakeUppercase{\romannumeral 1}.
The comparison involves binaries compiled with different compilers (i.e., Clang and GCC) and different optimization levels (i.e., {\tt O0}, {\tt O2}, and {\tt O3}).
To conduct the evaluation, we first use \toolname to sample each function in these binaries and aggregate the distribution of observable values. 
Then for each pair of comparison, we use functions compiled with higher-level optimizations to query the ones with lower optimization level. 
Specifically, for each function in the optimized binary, we compute its similarity score against all lower-optimized functions, and use the ones with the highest similarity scores to compute the PR@1. 
Besides PR@1, we also use PR@3 and @5 to compare with IMF for better illustrate the performance of \toolname.
We remove the results of functions with only 1 or 2 basic blocks since they are basically wrapper functions. 


The comparison results with IMF and BLEX are shown in Table~\ref{tab:baseline1}. The first column lists the compilers and the optimization flags used to generate the reference and query binaries.
The second column is the number of the functions that appear in both binaries. Note that some compiler optimizations, e.g., function inlining, remove functions from the binaries. 
Columns 3-5, 6-7, and 8-9 list PR@1, @3, and @5, respectively.
We present the results of \toolname{}, IMF, and BLEX from left to right for each metric.
Note that BLEX only reports the PR@1 and does not have results for binaries compiled with clang.
\toolname outperforms BLEX on PR@1 and outperforms IMF on all the 3 metrics under all the comparison settings. Especially, for function pairs from (clang-O0, gcc-O3) and (gcc-O0 and clang-O3), which are the most challenging settings in our experiment, \toolname outperforms IMF by about 10\%. 

\noindent{\bf Comparison to Baseline-\MakeUppercase{\romannumeral 2}. }To compare with Baseline-\MakeUppercase{\romannumeral 2}, we use Dataset-\MakeUppercase{\romannumeral 2}. We directly use the reported result on the How-Solve paper~\cite{How-Solve} for comparison because their code is currently unavailable. Following the setup of How-Solve paper, for each positive pair, we introduce 10 negative pairs to build up the test set. As Fig.~\ref{fig:how-help} illustrates, \toolname achieves scores from 0.76 to 0.99 on different programs, which is at least 10\% better than the How-Solve.















\subsection{RQ2: Performance Variations with Different Data Compositions}
\label{sec:eval:ratio}
In this section, we aim to analyze how different dataset compositions  affect the performance of different tools.
A dataset is composed of negative samples (dissimilar pairs) and positive samples (similar pairs). A class ratio N:1 means that for a query, apart from the ground truth target function, we also sample N of other functions as the negative data.

However, 5:1 is not realistic in real-world scenarios. A tool may need to compare a function with all the functions in a project to find the real similar one, which is the only true positive and all the other functions are true negatives. The ratio is usually very large. 
We argue our ratio around 1:1000 is more realistic.

We compute the PR@1 of \toolname, Trex and Safe with different ratio settings including 1:1, 5:1, 10:1, 20:1, 50:1, 100:1, 500:1, $\infty$:1. $\infty$ is the number of all the target functions in the project.

As Fig.~\ref{fig:baseline2-2} depicts, as the ratio increases, the PR@1 of all the tools decreases. \toolname degrades 9\% on GMP and 48\% on OpenSSL as the ratio increases from 1:1 to $\infty$:1. This reveals that it is more challenging to match similar functions with higher ratios.
For Coreutils, the precision of \toolname degrades 22\% as the ratio increases from 1:1 to $\infty$:1, whereas the precision of the other two tools degrades at least 64\%.
\toolname is hence more resilient to class ratio changes and likely performs better in real world scenarios.


\subsection{RQ3: Case Study}
The case study aims to show how our tool can discover 1-day vulnerabilities (CVEs) among a large amount of binaries. After a vulnerability is reported and confirmed, we have a vulnerable assembly function. A binary similarity tool can be used to search for vulnerable functions in real-world binaries.
We collect 10 1-day CVEs and  use the optimized version of the problematic function to search its counterpart in the unoptimized library.
The results show that our tool can find the ground truth function as the top one in most cases, while the other two ML-based methods can only find 1 of them, respectively. Even if we look into the top 30, both of them can only find 2 of these problematic functions.
Details can be found in our supplementary documents~\cite{sup-docs}. 

 



==> old-moti-code.tex <==



==> response-letter.tex <==




==> tab_config.tex <==
\begin{table}[t]
\footnotesize
    \caption{Perf. w.r.t. Different Configurations. The first two columns list the configurations we alter and the values we use for that configuration. Bold texts are default values for the related configurations. The remaining three columns list the PR@1, coverage for -O0 programs, and coverage for -O3 programs, respectively. The highest value for each column is marked as bold. %
    }
    \centering
    \begin{tabular}{rrccc}
    \toprule
      Configuration & Value & PR@1 & Cover-O0  & Cover-O3 \\ 
    \midrule
    \multirow{5}{*}{Loop-Unroll} & 1    & 0.828       & 0.963      & 0.887  \\
                                & 10    & {\bf 0.862}       & 0.979      & 0.955  \\
                                & {\bf 20}    & 0.857       & 0.980      & 0.955  \\
                                & 30    & 0.856       & 0.980      & 0.954  \\
                                & 40    & 0.853       & 0.980      & {\bf 0.956}  \\
    \midrule
    \multirow{5}{*}{String-Len} & 5    & 0.852       & 0.980      & 0.955  \\
                                & 10    & 0.856       & 0.980      & 0.955  \\
                                & 15    & 0.855       & 0.980      & 0.955  \\
                                & {\bf 20}    & 0.857       & 0.980      & 0.955  \\
                                & 25    & 0.856       & 0.980      & 0.954  \\
    \midrule
    \multirow{5}{*}{Mem-Size} & {\bf 64k}    & 0.853       & 0.979      & 0.952  \\
                                & 128k    & 0.850       & 0.979      & 0.952  \\
                                & 256k    & 0.850       & 0.979      & 0.953  \\
                                & 512k    & 0.855       & 0.978      & 0.953  \\
                                & 1MB    & 0.857       & 0.980      & 0.955  \\
    \midrule
    \multirow{5}{*}{Pred.-Instance} & {\bf 1}    & 0.857       & 0.980      & 0.955  \\
                                & 2    & 0.848       & 0.979      & 0.953  \\
                                & 3    & 0.849       & 0.979      & 0.954  \\
                                & 4    & 0.849       & 0.980      & 0.952  \\
                                & 5    & 0.850       & 0.979      & 0.952  \\
    \midrule
    \multirow{5}{*}{Input-Init} & {\bf Same}    & 0.857       & {\bf 0.981}     & 0.949  \\
                                & Rand1    & 0.845       & 0.980      & 0.950  \\
                                & Rand2    & 0.833       & 0.980      & 0.949  \\
                                & Rand3    & 0.841       & 0.980      & 0.949  \\
                                & Rand4    & 0.841       & 0.980      & 0.950  \\
    \bottomrule
    \end{tabular}
    \label{tab:config}
\end{table}

==> tab_cve.tex <==
\begin{table*}[t]
    \caption{Searching for One-Day Vulnerabilities. For each CVE-related function, we query with its optimized version in all the functions from the unoptimized binary. The first column lists the ID of CVE. Columns 2-4 show the project, the number of candidate functions, and the name of the problematic function. The last three columns show the ranking of similarity scores for the ground truth function generated by SAFE, Trex, and \toolname, respectively. An X means we do not find the problematic function within the top 200 matched functions. %
    }
    \centering
    \begin{tabular}{rlllllg}
    \toprule
         \multirow{2}{*}{CVE} & \multirow{2}{*}{Project} & \multirow{2}{*}{\#Func.} & \multirow{2}{*}{Func. Name} & \multicolumn{3}{c}{Result} \\
         \cmidrule(lr){5-7}
         & & & & SAFE & Trex & \cellcolor{white}\toolname \\
     \midrule
    CVE-2017-18018 & Coreutils & 931 & chown & 26 & X & 1\\
    CVE-2007-2452 & Findutils(locate) & 97 & visit\_old\_format & X & 5 & 1\\
    \midrule
    CVE-2021-20311 & \multirow{3}{*}{ImageMagick} & \multirow{3}{*}{1702} & sRGBTransformImage & X & X & 43\\
    CVE-2021-20309 &                             &  & WaveImage & 40 & X & 1\\
    CVE-2019-13308 &                             &  & ComplexImages & 73 & X & 1\\
    \midrule
    CVE-2016-9842 & Zlib & 91 & inflateMark & 34 & 1 & 1\\
    CVE-2021-4044 & Openssl & 2653 & X509\_verify\_cert & X & X & 1\\
    CVE-2021-3711 & Openssl & 2653 & EVP\_PKEY\_decrypt & 10 & X & 1\\
    \bottomrule
    \end{tabular}
    \label{tab:cve}
\end{table*}

==> tab_eva_baseline.tex <==
\newcommand{\problem}[1]{{\bf \color{red}#1}}
\definecolor{Gray}{gray}{0.85}
\newcolumntype{g}{>{\columncolor{Gray}}c}



\begin{table}[t]
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\caption{Comparison of \toolname, IMF, and BLEX. \textbf{\textit{C}} and \textbf{\textit{G}} denote Clang and GCC, respectively. Each precision is averaged over the 106 binaries in Coreutils.
}
\label{tab:baseline1}
\centering
\revise{
    \begin{tabular}{cgccgcgc}
    \toprule
    \multirow{2.5}{*}{Pair} & \multicolumn{3}{c}{Precision@1} & \multicolumn{2}{c}{Precision@3} & \multicolumn{2}{c}{Precision@5}\\
         \cmidrule(lr){2-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
         & \cellcolor{white}\toolname & IMF & BLEX & \cellcolor{white}\toolname & IMF & \cellcolor{white}\toolname & IMF\\
         \midrule
     \textbf{\textit{C}}-O0 \textbf{\textit{C}}-O3 
     & 94.5 & 77.5 & X & 98.2 & 84.2 & 98.7 & 86.4\\
     \textbf{\textit{C}}-O2 \textbf{\textit{C}}-O3 
     & 99.8 & 97.3 & X & 100.0 & 99.3 & 100.0 & 99.4\\
     \textbf{\textit{C}}-O0 \textbf{\textit{G}}-O3 
     & \textbf{94.5} & 60.1 & X & 97.3 & 70.6 & 98.6 & 73.4\\
     \textbf{\textit{G}}-O0 \textbf{\textit{G}}-O3 
     & 96.3 & 70.4 & 61.1 & 98.0 & 81.3 & 98.7 & 84.6\\
     \textbf{\textit{G}}-O2 \textbf{\textit{G}}-O3 
     & 98.6 & 89.5 & 77.1 & 99.4 & 95.5 & 99.8 & 96.2\\
     \textbf{\textit{G}}-O0 \textbf{\textit{C}}-O3 
     & \textbf{92.2} & 66.0 & X   & 94.1 & 76.1 & 96.2 & 80.0\\
     {\bf Average} & {\bf 96.0} & \textbf{76.8} & \textbf{69.1} & \textbf{97.8} & \textbf{84.5} & \textbf{98.7} & \textbf{86.7} \\ 
     \bottomrule
    \end{tabular}
    }
    \label{tab:my_label}
\end{table}






==> tab_eva_budget.tex <==
\begin{table}[t]
\footnotesize
    \caption{\revise{Perf. w.r.t. Different Budgets}
    }
    \centering
    \revise{
    \begin{tabular}{rccccccc}
    \toprule
     & 1 & 20 & 50 & 100 & 200 & 400 & 600\\ 
    \midrule
    PR@1        & 70    & 74    & 79    & 81    & 85    & 86    & 86 \\
    Cover-O0    & 63    & 87    & 91    & 94    & 96    & 98    & 98 \\
    Cover-O3    & 51    & 79    & 84    & 88    & 93    & 95    & 96 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-14pt}
    \label{tab:code-coverage}
\end{table}

==> tab_eva_memory_models.tex <==
\begin{table}[t!]
\footnotesize
    \caption{Perf. w.r.t. Different Memory Models}
    \centering
    \revise{
    \begin{tabular}{rccc}
    \toprule
     & No-Mem & Const & PMM \\ 
    \midrule
    PR@1        & 76.35    & 83.48    & {\bf 85.75}    \\
    Cover-O0    & 97.59    & 97.70    & {\bf 98.03}    \\
    Cover-O3    & 94.39   & 95.11    & {\bf 95.52}    \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:pmm}
\end{table}

==> tab_eva_path_sampling.tex <==
\begin{table}[t]
\footnotesize
    \caption{\revise{Perf. w.r.t. Different Path Sampling Strategies}}
    \centering
    \revise{
    \begin{tabular}{rccc}
    \toprule
     & LastPred & Det. & \toolname \\ 
    \midrule
    PR@1 & 40.24  & 79.27 & {\bf 91.46}  \\
    Cover-O0 & 66.28   & 96.77 & 96.81  \\
    Cover-O3 & 53.14   & 92.95 & 92.97  \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-14pt}
    \label{tab:path-sampling}
\end{table}

==> tab_multi_arch.tex <==
\begin{table}[H]
    \caption{\revise{Cross-architecture Performance on Coreutils. The first column lists the  configurations used to compile the binary files in comparison. \textbf{\textit{X}} and \textbf{\textit{A}} denote X86-64 and AArch 64, respectively. For each row, we use the functions in the binary compiled by the second option to query the similar function in the first binary. The second column lists the precision.}
    }
    \centering
    \revise{
    \begin{tabular}{rccc}
    \toprule
    Pair & PR@1 \\ 
    \midrule
    \textbf{\textit{X}}-O0 \textbf{\textit{X}}-O3 & 89.4\\
    \textbf{\textit{A}}-O0 \textbf{\textit{A}}-O3 & 86.8\\
    \textbf{\textit{X}}-O0 \textbf{\textit{A}}-O3 & 81.2\\
    \textbf{\textit{A}}-O0 \textbf{\textit{X}}-O3 & 81.5\\
    \textbf{\textit{X}}-O0 \textbf{\textit{A}}-O0 & 84.9\\
    \textbf{\textit{X}}-O3 \textbf{\textit{A}}-O3 & 83.9\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:multi-arch}
\end{table}

==> tab_statistics.tex <==
\begin{table}[t]
    \centering
    \caption{\revise{Statistics of Dataset. The first two columns are the names of projects and optimization flags used to compile the binary files. The 3-4 columns are the functions and the number of basic blocks in the related binary files. Note that we remove functions with no more than 3 basic blocks since they are basically wrapper functions.%
    }}
    \revise{
    \label{tab:dataset-stats}
    \begin{tabular}{rcrr}
    \toprule
    Name & Opt. & \#Func. & \#B.B.\\
    \midrule
    \multirow{3}{*}{Coreutils-GCC} & O0 & 1943 & 40096 \\
                               & O2 & 1179 & 36318 \\
                               & O3 & 1081 & 42467 \\
   \midrule
    \multirow{3}{*}{Coreutils-Clang} & O0 & 1912 & 52340 \\                               
                               & O2 & 999 & 39099 \\
                               & O3 & 978 & 41816 \\
   \midrule
\multirow{3}{*}{Curl} & O0 & 774 & 17660 \\                               
                               & O2 & 517 & 14514 \\
                               & O3 & 469 & 17102 \\
\midrule
\multirow{3}{*}{ImageMagick} & O0 & 2849 & 102163 \\                               
                               & O2 & 1883 & 103689 \\
                               & O3 & 1817 & 121472 \\
\midrule
\multirow{3}{*}{Diffutils} & O0 & 609 & 12266 \\                               
                               & O2 & 407 & 11540 \\
                               & O3 & 412 & 14298 \\
\midrule
\multirow{3}{*}{Findutils} & O0 & 955 & 18769 \\                               
                               & O2 & 621 & 16212 \\
                               & O3 & 616 & 21943 \\
\midrule
\multirow{3}{*}{OpenSSL} & O0 & 3572 & 68022 \\                               
                               & O2 & 2941 & 58291 \\
                               & O3 & 3054 & 75529 \\
\midrule
\multirow{3}{*}{Zlib} & O0 & 118 & 2779 \\                               
                               & O2 & 106 & 2627 \\
                               & O3 & 98 & 3926 \\
\midrule
\multirow{3}{*}{GMP} & O0 & 605 & 12695 \\                               
                               & O2 & 537 & 14195 \\
                               & O3 & 526 & 16150 \\
\midrule
\multirow{3}{*}{SQLite} & O0 & 1513 & 28224 \\                               
                               & O2 & 1071 & 30636 \\
                               & O3 & 984 & 40171 \\
\midrule
Total & - & {\bf 35146} & {\bf 1077k}\\
\bottomrule
   
    \end{tabular}
    }
\end{table}
